Deep Learning Library Testing: Definition, Methods and Challenges

In recent years, software systems powered by deep learning (DL) techniques have significantly facilitated people's lives in many aspects. As the backbone of these DL systems, various DL libraries undertake the underlying optimization and computation. However, like traditional software, DL libraries are not immune to bugs, which can pose serious threats to users' personal property and safety. Studying the characteristics of DL libraries, their associated bugs, and the corresponding testing methods is crucial for enhancing the security of DL systems and advancing the widespread application of DL technology. This paper provides an overview of the testing research related to various DL libraries, discusses the strengths and weaknesses of existing methods, and provides guidance and reference for the application of the DL library. This paper first introduces the workflow of DL underlying libraries and the characteristics of three kinds of DL libraries involved, namely DL framework, DL compiler, and DL hardware library. It then provides definitions for DL underlying library bugs and testing. Additionally, this paper summarizes the existing testing methods and tools tailored to these DL libraries separately and analyzes their effectiveness and limitations. It also discusses the existing challenges of DL library testing and outlines potential directions for future research.

==> bib.tex <==
\begin{thebibliography}{99}
    % Author A, Author B, Author C. Reference title. Journal, Year, Vol: Number or pages
    % Author A, Author B, Author C, et al. Reference title. In: Proceedings of Conference, Place, Year. Number or pages
% \bibitem{abadi2016tensorflow} Abadi M, Barham P, Chen J, et al. Tensorflow: a system for large-scale machine learning. In: 12th {USENIX} Symposium on Operating Systems Design and Implementation(OSDI), Savannah, 2016. 265-283.

% \bibitem{lecun2015deep} LeCun Y, Bengio Y, Hinton G. Deep learning. Nature, 2015. 521: 436-444.

% \bibitem{guo2020audee}Guo Q, Xie X, Li Y, et al. Audee: Automated testing for deep learning frameworks. In: Proceedings of the 35th IEEE/ACM International Conference on Automated Software Engineering(ICSE), Melbourne, 2020. 486-498.


% =========================== section1 =========================== 
\bibitem{tesla1pytorch} Sun Y. Tesla and Pytorch — Pytorch Developer Conference Highlights Part. Available from: https://medium.com/data-science-bootcamp/tesla-and-pytorch-pytorch-developer-conference-highlights-part-3ed36f2c9d5e

\bibitem{google1tensorflow} TensorFlow. Learn how TensorFlow solves real, everyday machine learning problems. Available from: https://www.tensorflow.org/about/case-studies.

\bibitem{pham2019cradle} Pham H V, Lutellier T, Qi W, et al. CRADLE: cross-backend validation to detect and localize bugs in deep learning libraries. In: 2019 IEEE/ACM 41st International Conference on Software Engineering (ICSE), Montreal, Canada, 2019. 1027-1038.

\bibitem{wei2022free} Wei A J, Deng Y L, Yang C Y, et al. Free lunch for testing: Fuzzing deep-learning libraries from open source. In: Proceedings of the 44th International Conference on Software Engineering, Pittsburgh, USA, 2022. 995-1007.

\bibitem{teslacase} Ken K. Exclusive: surveillance footage of tesla crash on sf's bay bridge hours after elon musk announces “self-driving” feature. Available from: https://theintercept.com/2023/01/10/tesla-crash-footage-autopilot/

\bibitem{ubercase} ABC7.com staff. Uber gives up testing of self-driving cars in California in wake of fatal Arizona crash. Available from: https://abc7.com/self-driving-uber-crash-video-pedestrian-hit-by-car-autonomous-vehicles/3269690/

\bibitem{deng2022fuzzing} Deng Y L, Yang C Y, Wei A J, et al. Fuzzing deep-learning libraries via automated relational API inference. In: Proceedings of the 30th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering, Singapore, Singapore, 2022. 44-56.

\bibitem{usnaiia} Office of Science and Technology Policy. National Artificial Intelligence Initiative Act of 2020. Available from: https://www.ai.gov/wp-content/uploads/2023/04/National-Artificial-Intelligence-Initiative-Act-of-2020.pdf

\bibitem{euaiact} European Commission. Artificial Intelligence Act. Available from: https://artificialintelligenceact.eu/wp-content/uploads/2021/08/The-AI-Act.pdf

\bibitem{zhang2020machine} Zhang J M, Harman M, Ma L, et al. Machine learning testing: Survey, landscapes and horizons. IEEE Transactions on Software Engineering, 2020, 48: 1-36.

\bibitem{ma2023survey} Ma X Y, Du X T, Cai Q, et al. A Survey on Testing of Deep Learning Frameworks (in Chinese). Journal of Software, 2023.

\bibitem{li2020deep} Li M Z, Liu Y, Liu X Y, et al. The deep learning compiler: A comprehensive survey. IEEE Transactions on Parallel and Distributed Systems, 2020, 32: 708-727.

\bibitem{braiek2020testing} Braiek H B, Khomh F. On testing machine learning programs. Journal of Systems and Software, 2020, 164: 110542.

\bibitem{gezici2022systematic} Gezici B, Tarhan A K. Systematic literature review on software quality for AI-based software. Empirical Software Engineering, 2022, 27: 66.

\bibitem{martinez2022software} Martínez-Fernández S, Bogner J, Franch X, et al. Software engineering for AI-based systems: a survey. ACM Transactions on Software Engineering and Methodology (TOSEM), 2022, 31: 1-59.
% the challenge and limitation about using SE knowledge to improve AI system. focus on system safety and reliability, not testing DL libs

\bibitem{zhang2022testing} Zhang X Y, Shen C, Lin C H, et al. The Testing and Repairing Methods for Machine Learning Model Security (in Chinese). ACTA ELECTONICA SINICA, 2022, 50: 2884.
%  AI based software quality evaluation, not testing DL libs

% =========================== section2 =========================== 

\bibitem{abadi2016tensorflow} Abadi M. TensorFlow: learning functions at scale. In: Proceedings of the 21st ACM SIGPLAN International Conference on Functional Programming, Nara, Japan, 2016. 1-1.

\bibitem{paszke2019pytorch} Paszke A, Gross S, Massa F, et al. Pytorch: An imperative style, high-performance deep learning library. Advances in neural information processing systems, 2019. 8024-8035.

% \bibitem{ma2019paddlepaddle} Ma Y, Yu D, Wu T, et al. PaddlePaddle: An open-source deep learning platform from industrial practice. Frontiers of Data and Computing, 2019, 1: 105-115.

\bibitem{ONNX} Microsoft. ONNX Github repository. 2023. https://github.com/onnx/onnx. Accessed May 20, 2023

\bibitem{rotem2018glow} Rotem N, Fix J, Abdulrasool S, et al. Glow: Graph lowering compiler techniques for neural networks. arXiv preprint arXiv:1805.00907, 2018.

\bibitem{chen2018tvm} Chen T Q, Moreau T, Jiang Z H, et al. TVM: An automated end-to-end optimizing compiler for deep learning. In: 13th USENIX Symposium on Operating Systems Design and Implementation, Carlsbad, USA, 2018. 578-594.

% \bibitem{XLA} OpenXLA. OpenXLA Github repository. 2023. https://github.com/openxla/xla. Accessed May 20, 2023

\bibitem{chetlur2014cudnn} Chetlur S, Woolley C, Vandermersch P, et al. cudnn: Efficient primitives for deep learning. arXiv preprint arXiv:1410.0759, 2014.

\bibitem{ignatov2018ai} Ignatov A, Timofte R, Chou W, et al. Ai benchmark: Running deep neural networks on android smartphones. In: Proceedings of the European Conference on Computer Vision (ECCV) Workshops, Munich, Germany, 2018, 288--314.

\bibitem{IEEEstdBug} IEEE Standards Association. Ieee standard classification for software anomalies. IEEE Computer Society, 2009.

\bibitem{islam2019comprehensive} Islam M J, Nguyen G, Pan R, et al. A comprehensive study on deep learning bug characteristics. In: Proceedings of the 2019 27th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering, Tallinn, Estonia, 2019. 510-520.

\bibitem{yang2022comprehensive} Yang Y L, He T X, Xia Z L, et al. A comprehensive empirical study on bug characteristics of deep learning frameworks. Information and Software Technology, 2022, 151: 107004.

\bibitem{chen2022toward} Chen J J, Liang Y H, Shen Q C, et al. Toward understanding deep learning framework bugs. ACM Transactions on Software Engineering and Methodology, 2022.

\bibitem{shen2021comprehensive} Shen Q C, Ma H Y, Chen J J, et al. A comprehensive study of deep learning compiler bugs. In: Proceedings of the 29th ACM Joint meeting on european software engineering conference and symposium on the foundations of software engineering, Athens, Greece, 2021. 968-980.

\bibitem{liu2022coverage} Liu J W, Wei Y X, Yang S, et al. Coverage-guided tensor compiler fuzzing with joint ir-pass mutation. Proceedings of the ACM on Programming Languages, 2022, 6: 1-26.

\bibitem{xiao2022metamorphic} Xiao D W, Liu Z B, Yuan Y Y, et al. Metamorphic testing of deep learning compilers. Proceedings of the ACM on Measurement and Analysis of Computing Systems, 2022, 6: 1-28.

\bibitem{uezono2022achieving} Uezono T, He Y, Li Y. Achieving automotive safety requirements through functional in-field self-test for deep learning accelerators. In: 2022 IEEE International Test Conference (ITC), Anaheim, USA, 2022. 465-473.

\bibitem{wang2020accuracy} Wang C J, Shen J, Fang C R, et al. Accuracy measurement of deep neural network accelerator via metamorphic testing. In: 2020 IEEE International Conference On Artificial Intelligence Testing (AITest), Oxford, UK, 2020. 55-61.

\bibitem{nistor2015caramel} Nistor A, Chang P C, Radoi C, et al. Caramel: Detecting and fixing performance problems that have non-intrusive fixes. In: 2015 IEEE/ACM 37th IEEE International Conference on Software Engineering, Florence, Italy, 2015. 902-912.

\bibitem{jin2012understanding} Jin G L, Song L H, Shi X M, et al. Understanding and detecting real-world performance bugs. ACM SIGPLAN Notices, 2012, 47: 77-88.

\bibitem{patterson2021carbon} Patterson D A, Gonzalez J, Le Q V, et al. Carbon emissions and large neural network training. arXiv preprint arXiv:2104.10350, 2021.

\bibitem{guo2019empirical} Guo Q Y, Chen S, Xie X F, et al. An empirical study towards characterizing deep learning development and deployment across different frameworks and platforms. In: 2019 34th IEEE/ACM International Conference on Automated Software Engineering (ASE), San Diego, USA, 2019. 810-822.


\bibitem{levental2020comparing} Levental M, Orlova E. Comparing the costs of abstraction for dl frameworks. arXiv preprint arXiv:2012.07163, 2020.

\bibitem{mckeeman1998differential} McKeeman W M. Differential testing for software. Digital Technical Journal, 1998, 10: 100-107.

\bibitem{groce2007randomized} Groce A, Holzmann G, Joshi R. Randomized differential testing as a prelude to formal verification. In: 29th International Conference on Software Engineering (ICSE). Minneapolis, USA, 2007. 621-631.

\bibitem{wang2021qdiff} Wang J Y, Zhang Q, Xu G H, et al. QDiff: Differential testing of quantum software stacks. In: 2021 36th IEEE/ACM International Conference on Automated Software Engineering (ASE). Melbourne, Australia, 2021. 692-704.

\bibitem{guo2020audee} Guo Q Y, Xie X F, Li Y, et al. Audee: Automated testing for deep learning frameworks. In: Proceedings of the 35th IEEE/ACM International Conference on Automated Software Engineering(ASE), Melbourne, Australia, 2020. 486-498.

\bibitem{liang2018fuzz} Liang J, Wang M, Chen Y, et al. Fuzz testing in practice: Obstacles and solutions. In: 2018 IEEE 25th International Conference on Software Analysis, Evolution and Reengineering (SANER), Campobasso, Italy, 2018. 562-566.

\bibitem{manes2019art} Manès V J M, Han H S, Han C, et al. The art, science, and engineering of fuzzing: A survey. IEEE Transactions on Software Engineering, 2019, 47: 2312-2331.

\bibitem{liu2012software} Liu B, Shi L, Cai Z, et al. Software vulnerability discovery techniques: A survey. In: 2012 fourth international conference on multimedia information networking and security, Washington, United States, 2012. 152-156.

\bibitem{oehlert2005violating} Oehlert P. Violating assumptions with fuzzing. IEEE Security \& Privacy, 2005, 3: 58-62.

\bibitem{deng2023fuzzing} Deng Y L, Xia C S, Peng H R, et al. Large Language Models are Zero-Shot Fuzzers: Fuzzing Deep-Learning Libraries via Large Language Models. In: Proceedings of the 32nd ACM SIGSOFT International Symposium on Software Testing and Analysis (ISSTA 2023). Seattle, United States, 2023.

\bibitem{xie2022docter} Xie D N, Li Y T, Kim M, et al. DocTer: documentation-guided fuzzing for testing deep learning API functions. In: Proceedings of the 31st ACM SIGSOFT International Symposium on Software Testing and Analysis, Virtual Event, South Korea, 2022. 176-188.

\bibitem{chen1998metamorphic} Chen T Y, Cheung S, Yiu S M. Metamorphic testing: a new approach for generating next test cases. technical report hkust-cs98-01. Hong Kong Univ. of Science and Technology, 1998.

\bibitem{segura2016survey} Segura S, Fraser G, Sanchez A B, et al. A survey on metamorphic testing. IEEE Transactions on software engineering, 2016, 42: 805-824.
 
\bibitem{zhang2021autotrainer} Zhang X Y, Zhai J, Ma S Q, et al. Autotrainer: An automatic dnn training problem detection and repair system. In: 2021 IEEE/ACM 43rd International Conference on Software Engineering (ICSE), Madrid, Spain, 2021. 359-371.

\bibitem{udeshi2018automated} Udeshi S, Arora P, Chattopadhyay S. Automated directed fairness testing. In: Proceedings of the 33rd ACM/IEEE International Conference on Automated Software Engineering, Montpellier, France, 2018. 98-108.


% =========================== section3 =========================== 
% table 1
\bibitem{wang2022eagle} Wang J N, Lutellier T, Qian S S, et al. EAGLE: creating equivalent graphs to test deep learning libraries. In: Proceedings of the 44th International Conference on Software Engineering, Pittsburgh, USA, 2022. 798-810.

\bibitem{schumi2022exais} Schumi R, Sun J. ExAIS: executable AI semantics. In: Proceedings of the 44th International Conference on Software Engineering, Pittsburgh, USA, 2022. 859-870.

\bibitem{li2023comet} Li M Z, Cao J L, Tian Y Q, et al. COMET: Coverage-guided Model Generation For Deep Learning Library Testing. ACM Transactions on Software Engineering and Methodology, 2023.

\bibitem{ding2017validating} Ding J H, Kang X J, Hu X H. Validating a deep learning framework by metamorphic testing. In: 2017 IEEE/ACM 2nd International Workshop on Metamorphic Testing (MET), Buenos Aires, Argentina, 2017. 28-34.

\bibitem{christou2022ivysyn} Christou N, Jin D, Atlidakis V, et al. IvySyn: Automated Vulnerability Discovery in Deep Learning Frameworks. In: Proceedings of the 32nd USENIX Security Symposium (USENIX Sec'23), Anaheim, USA. 2023.
% end table 1

\bibitem{zhang2018empirical} Zhang Y H, Chen Y F, Cheung S C, et al. An empirical study on TensorFlow program bugs. In: Proceedings of the 27th ACM SIGSOFT International Symposium on Software Testing and Analysis, Amsterdam, The Netherlands, 2018. 129-140.

\bibitem{zhang2020empirical} Zhang R, Xiao W C, Zhang H Y, et al. An empirical study on program failures of deep learning jobs. In: Proceedings of the ACM/IEEE 42nd International Conference on Software Engineering, Seoul, South Korea, 2020. 1159-1170.

\bibitem{zhang2019software} Zhang X F, Yang Y L, Feng Y, et al. Software engineering practice in the development of deep learning applications. arXiv preprint arXiv:1910.03156, 2019.

\bibitem{Chen2020comprehensive} Chen Z P, Cao Y B, Liu Y Q, et al. A comprehensive study on challenges in deploying deep learning based software. In: Proceedings of the 28th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering, Virtual Event, USA, 2020. 750-762.


% study


\bibitem{wang2020deep} Wang Z, Yan M, Chen J J, et al. Deep learning library testing via effective model generation. In: Proceedings of the 28th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering, Virtual Event, USA, 2020. 788-799.

\bibitem{jia2022injected} Jia L, Zhong H, Wang X Y, et al. How Do Injected Bugs Affect Deep Learning?. In: 2022 IEEE International Conference on Software Analysis, Evolution and Reengineering (SANER), Honolulu, USA, 2022. 793-804.


\bibitem{quan2022towards} Quan L L, Guo Q Y, Xie X F, et al. Towards Understanding the Faults of JavaScript-Based Deep Learning Systems. In: 37th IEEE/ACM International Conference on Automated Software Engineering, Rochester, USA, 2022. 1-13.

\bibitem{Aach2023large} Aach M, Inanc E, Sarma R, et al. Large scale performance analysis of distributed deep learning frameworks for convolutional neural networks. Journal of Big Data, 2023, 10: 1-23.

\bibitem{cao2022understanding} Cao J M, Chen B H, Sun C, et al. Understanding performance problems in deep learning systems. In: Proceedings of the 30th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering, Singapore, Singapore, 2022. 357-369.

\bibitem{liu2022taxonomy} Liu Z H, Zheng Y, Du X T, et al. Taxonomy of Aging-related Bugs in Deep Learning Libraries. In: 2022 IEEE 33rd International Symposium on Software Reliability Engineering (ISSRE), Charlotte, USA, 2022. 423-434.

\bibitem{du2022empirical} Du X T, Sui Y L, Liu Z H, et al. An empirical study of fault triggers in deep learning frameworks. IEEE Transactions on Dependable and Secure Computing, 2022.

\bibitem{harzevili2022characterizing} Harzevili N S, Shin J, Wang J J, et al. Characterizing and Understanding Software Security Vulnerabilities in Machine Learning Libraries. arXiv preprint arXiv:2203.06502, 2022.

% differential testing
\bibitem{liu2018benchmarking} Liu L, Wu Y Z, Wei W Q, et al. Benchmarking deep learning frameworks: Design considerations, metrics and beyond. In: 2018 IEEE 38th International Conference on Distributed Computing Systems (ICDCS), Vienna, Austria, 2018. 1258-1269.

\bibitem{ketkar2017introduction} Ketkar N, Ketkar N. Introduction to keras. Deep learning with python: a hands-on introduction, 2017, 97-111.

\bibitem{gu2022muffin} Gu J Z, Luo X H, Zhou Y F, et al. Muffin: Testing deep learning libraries via neural architecture fuzzing. In: Proceedings of the 44th International Conference on Software Engineering, Pittsburgh, USA, 2022. 1418-1430.

\bibitem{zhang2021predoo} Zhang X, Sun N, Fang C, et al. Predoo: precision testing of deep learning operators. In: Proceedings of the 30th ACM SIGSOFT International Symposium on Software Testing and Analysis, Virtual Event, Denmark, 2021. 400-412.

\bibitem{zhang2021duo} Zhang X F, Liu J W, Sun N, et al. Duo: Differential fuzzing for deep learning operators. IEEE Transactions on Reliability, 2021, 70: 1671-1685.

\bibitem{gu2022defect} Gu D D, Shi Y N, Liu X Z, et al. Defect Detection for Deep Learning Frameworks Based on Meta Operators (in Chinese). Chinese Journal Of Computers, 2022, 45: 240-255.

\bibitem{prochnow2022diffwatch} Prochnow A, Yang J Q. DiffWatch: watch out for the evolving differential testing in deep learning libraries. In: Proceedings of the ACM/IEEE 44th International Conference on Software Engineering: Companion Proceedings, Pittsburgh, USA, 2022. 46-50.

\bibitem{chen2021evaluating} Chen M, Tworek J, Jun H, et al. Evaluating large language models trained on code. arXiv preprint arXiv:2107.03374, 2021.

\bibitem{fried2022incoder} Fried D, Aghajanyan A, Lin J, et al. Incoder: A generative model for code infilling and synthesis. arXiv preprint arXiv:2204.05999, 2022.

\bibitem{deng2023large} Deng Y L, Xia C S, Yang C Y, et al. Large language models are edge-case fuzzers: Testing deep learning libraries via fuzzgpt. arXiv preprint arXiv:2304.02014, 2023.

\bibitem{nijkamp2022codegen} Nijkamp E, Pang B, Hayashi H, et al. Codegen: An open large language model for code with multi-turn program synthesis. arXiv preprint arXiv:2203.13474, 2022.

\bibitem{yang2023fuzzing} Yang C Y, Deng Y L, Yao J Y, et al. Fuzzing automatic differentiation in deep-learning libraries. arXiv preprint arXiv:2302.04351, 2023.

\bibitem{davis1981pseudo} Davis M D, Weyuker E J. Pseudo-oracles for non-testable programs. In: Proceedings of the ACM'81 Conference, Los Angeles, USA, 1981. 254-257.

\bibitem{shi2023acetest} Shi J Y, Xiao Y, Li Y K, et al. ACETest: Automated Constraint Extraction for Testing Deep Learning Operators. In: Proceedings of the 32nd ACM SIGSOFT International Symposium on Software Testing and Analysis (ISSTA 2023), Seattle, United States, 2023.

\bibitem{kang2022skipfuzz} Kang H J, Rattanukul P, Haryono S A, et al. SkipFuzz: Active Learning-based Input Selection for Fuzzing Deep Learning Libraries. arXiv preprint arXiv:2212.04038, 2022.

\bibitem{liu2023neuri} Liu J, Peng J, Wang Y, et al. Neuri: Diversifying dnn generation via inductive rule inference. arXiv preprint arXiv:2302.02261, 2023.

\bibitem{li2022mmos} Li J Q, Li S Y, Wu J W, et al. MMOS: Multi-Staged Mutation Operator Scheduling for Deep Learning Library Testing. In: GLOBECOM 2022-2022 IEEE Global Communications Conference, Rio de Janeiro, Brazil, 2022. 6103-6108.

\bibitem{zou2023deep} Zou Y L, Sun H F, Fang C R, et al. Deep learning framework testing via hierarchical and heuristic model generation. Journal of Systems and Software, 2023, 201: 111681.

\bibitem{li2023starcoder} Li R, Allal L B, Zi Y, et al. StarCoder: may the source be with you!. arXiv preprint arXiv:2305.06161, 2023.

\bibitem{xie2009application} Xie X, Ho J, Murphy C, et al. Application of metamorphic testing to supervised classifiers. In: 2009 Ninth International Conference on Quality Software, Jeju, Korea, 2009. 135-144.

\bibitem{murphy2009using} Murphy C, Shen K, Kaiser G. Using JML runtime assertion checking to automate metamorphic testing i applications without test oracles. In: 2009 International Conference on Software Testing Verification and Validation, Denver, USA, 2009. 436-445.

\bibitem{xie2011testing} Xie X Y, Ho J W K, Murphy C, et al. Testing and validating machine learning classifiers by metamorphic testing. Journal of Systems and Software, 2011, 84: 544-558.

\bibitem{dwarakanath2018identifying} Dwarakanath A, Ahuja M, Sikand S, et al. Identifying implementation bugs in machine learning based image classifiers using metamorphic testing. In: Proceedings of the 27th ACM SIGSOFT International Symposium on Software Testing and Analysis, Amsterdam, The Netherlands, 2018. 118-128.

\bibitem{zhang2021deepbackground} Zhang Z Y, Wang P, Guo H J, et al. DeepBackground: Metamorphic testing for Deep-Learning-driven image recognition systems accompanied by Background-Relevance. Information and Software Technology, 2021, 140: 106701.

\bibitem{herbold2022smoke} Herbold S, Haar T. Smoke testing for machine learning: simple tests to discover severe bugs. Empirical Software Engineering, 2022, 27: 45.

\bibitem{ge2023justintime} Ge J, Yu H Q, Fan G S, et al. Just-In-Time Defect Prediction for Intelligent Computing Frameworks (in Chinese). Journal of Software, 2023, 34: 0-0.


\bibitem{kim2021denchmark} Kim M, Kim Y, Lee E. Denchmark: A bug benchmark of deep learning-related software. In: 2021 IEEE/ACM 18th International Conference on Mining Software Repositories (MSR), Madrid, Spain, 2021. 540-544.

% % =========================== section4 =========================== 

\bibitem{wu23jitfuzz} Wu M Y, Lu M H, Cui H M, et al. Jitfuzz: Coverage-guided fuzzing for jvm just-in-time compilers. In: Proceedings of the 45th International Conference on Software Engineering, Melbourne, Australia. 2023.

\bibitem{tao2010automatic} Tao Q M, Wu W, Zhao C, et al. An automatic testing approach for compiler based on metamorphic testing technique. In: 2010 Asia Pacific Software Engineering Conference, Sydney, Australia, 2010. 270-279.

\bibitem{zhong2022enriching} Zhong H. Enriching Compiler Testing with Real Program from Bug Report. In: 37th IEEE/ACM International Conference on Automated Software Engineering, Rochester, USA, 2022. 40: 1-12.

\bibitem{chen2022boosting} Chen J J, Suo C Y. Boosting compiler testing via compiler optimization exploration. ACM Transactions on Software Engineering and Methodology (TOSEM), 2022, 31: 1-33.

\bibitem{chen2023compiler} Chen J J, Suo C Y, Jiang J J, et al. Compiler Test-Program Generation via Memoized Configuration Search. In: Proceedings of the 45th IEEE/ACM International Conference on Software Engineering, Melbourne, Australia, 2023.

\bibitem{liu2023nnsmith} Liu J, Lin J, Ruffy F, et al. Nnsmith: Generating diverse and valid test cases for deep learning compilers. In: Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems, Volume 2, Vancouver, Canada, 2023. 530-543.

\bibitem{du2021empirical} Du X, Zheng Z, Ma L, et al. An Empirical Study on Common Bugs in Deep Learning Compilers. In: 2021 IEEE 32nd International Symposium on Software Reliability Engineering (ISSRE), Wuhan, China, 2021. 184-195.

\bibitem{ren2023effective} Ren L Y, Wang Z H, Xiong Y F, et al. Effective Random Test Generation for Deep Learning Compilers. arXiv preprint arXiv:2302.00842, 2023.


\bibitem{yang2011finding} Yang X J, Chen Y, Eide E, et al. Finding and understanding bugs in C compilers. In: Proceedings of the 32nd ACM SIGPLAN conference on Programming language design and implementation, San Jose, USA, 2011. 283-294.

\bibitem{holler2012fuzzing} Holler C, Herzig K, Zeller A. Fuzzing with code fragments. In: 21st USENIX Security Symposium (USENIX Security 12), Bellevue, USA, 2012. 445-458.

\bibitem{ma2023fuzzing} Ma H Y, Shen Q C, Tian Y Q, et al. Fuzzing Deep Learning Compilers with HirGen. In: Proceedings of the 32nd ACM SIGSOFT International Symposium on Software Testing and Analysis (ISSTA 2023). Seattle, United States, 2023.

\bibitem{li2022alphaprog}  Li X T, Liu X, Chen L W, et al. ALPHAPROG: reinforcement generation of valid programs for compiler fuzzing. In: Proceedings of the AAAI Conference on Artificial Intelligence, Virtual Event, 2022. 36(11), 12559-12565.
 
% % =========================== section5 =========================== 

\bibitem{he2021efficient} He Y, Uezono T, Li Y. Efficient functional in-field self-test for deep learning accelerators. In: 2021 IEEE International Test Conference (ITC), Anaheim, USA, 2021. 93-102.

\bibitem{jorda2019performance} Jorda M, Valero-Lara P, Pena A J. Performance evaluation of cudnn convolution algorithms on nvidia volta gpus. IEEE Access, 2019, 7: 70461-70473.

\bibitem{nazir2023interpretable} Nazir Z, Yarovenko V, Park J G. Interpretable ML enhanced CNN Performance Analysis of cuBLAS, cuDNN and TensorRT. In: Proceedings of the 38th ACM/SIGAPP Symposium on Applied Computing, Tallinn, Estonia, 2023. 1260-1265.

\bibitem{kundu2021toward} Kundu S, Banerjee S, Raha A, et al. Toward functional safety of systolic array-based deep learning hardware accelerators. IEEE Transactions on Very Large Scale Integration (VLSI) Systems, 2021, 29: 485-498.

\bibitem{chaudhuri2022functional} Chaudhuri A, Talukdar J, Su F, et al. Functional criticality analysis of structural faults in AI accelerators. IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems, 2022, 41: 5657-5670.

\bibitem{kundu2023trouble} Kundu S, Banerjee S, Raha A, et al. Trouble-shooting at GAN Point: Improving Functional Safety in Deep Learning Accelerators. IEEE Transactions on Computers, 2023, 72: 2194-2208.

\bibitem{chaudhuri2023functional} Chaudhuri A, Chen C Y, Talukdar J, et al. Functional Test Generation for AI Accelerators using Bayesian Optimization*. In: 2023 IEEE 41st VLSI Test Symposium (VTS), San Diego, USA, 2023. 1-6.

\bibitem{buber2018performance} Buber E, Banu D. Performance analysis and CPU vs GPU comparison for deep learning. In: 2018 6th International Conference on Control Engineering \& Information Technology (CEIT), Istanbul, Turkey, 2018. 1-6.

\bibitem{liu2022tbem} Liu H Y, Liu S Y, Wen C L, et al. TBEM: Testing-Based GPU-Memory Consumption Estimation for Deep Learning. IEEE Access, 2022, 10: 39674-39680.

\bibitem{huang2022demystifying} Huang K F, Chen B H, Wu S S, et al. Demystifying Dependency Bugs in Deep Learning Stack. arXiv preprint arXiv:2207.10347, 2022.

\bibitem{lidbury2015many} Lidbury C, Lascu A, Chong N, et al. Many-core compiler fuzzing. ACM SIGPLAN Notices, 2015, 50: 65-76.

\bibitem{jiang2020cudasmith} Jiang B, Wang X, Chan W K, et al. Cudasmith: A fuzzer for CUDA compilers. In: 2020 IEEE 44th Annual Computers, Software, and Applications Conference (COMPSAC), Madrid, Spain, 2020. 861-871.
% % =========================== section6 =========================== 

\bibitem{just2014defects4j} Just R, Jalali D, Ernst M D. Defects4J: A database of existing faults to enable controlled testing studies for Java programs. In: Proceedings of the 2014 international symposium on software testing and analysis, San Jose, USA, 2014. 437-440.

\bibitem{sun2022causality} Sun B, Sun J, Pham L H, et al. Causality-based neural network repair. In: Proceedings of the 44th International Conference on Software Engineering, Pittsburgh, USA, 2022. 338-349.

\bibitem{li2021fault} Li Y, Wang S, Nguyen T. Fault localization with code coverage representation learning. In: 2021 IEEE/ACM 43rd International Conference on Software Engineering (ICSE), Madrid, Spain, 2021. 661-673.

\bibitem{meng2022improving} Meng X, Wang X, Zhang H, et al. Improving fault localization and program repair with deep semantic features and transferred knowledge. In: Proceedings of the 44th International Conference on Software Engineering, Pittsburgh, USA, 2022. 1169-1180.

\end{thebibliography}

==> tex/ack.tex <==
%!TEX root = ../main.tex


\Acknowledgements{This work was supported by National Natural Science Foundation of China (Grant Nos. 00000000 and 11111111).}

==> tftex/overview24.tex <==
\begin{table*}[]
\caption{DL Library Testing vs. DL Model Testing}
\label{tab:compiler_compare}
\centering
\footnotesize
\tabcolsep=5pt
\begin{tabular}{ccccc}
\toprule
& Test Input & Test Object & Test Property & Test Oracle \\ \midrule
\begin{tabular}[c]{@{}c@{}}DL   Library\\      Testing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Seceral lines of code to\\ call DL libray APIs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Program bugs in\\the DL library\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mainly correctness and   efficiency\\      of the DL library\end{tabular} & \begin{tabular}[c]{@{}c@{}}Difficult to construct   test\\      oracles in bug detection\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}DL   Model\\      Testing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Image, text, or\\ matrix data\end{tabular} & \begin{tabular}[c]{@{}c@{}}Secure problems on \\      DL model properties\end{tabular} & \begin{tabular}[c]{@{}c@{}}Correctness, robustness, interpretability, \\ efficiency, etc. of the DL model\end{tabular} & \begin{tabular}[c]{@{}c@{}}Metrics existing for testing   \\      and detecting problems\end{tabular} \\ \bottomrule
\end{tabular}
% \vspace{-10pt}
\end{table*}

==> tftex/seca_fig1.tex <==
% \begin{figure}
%     \centering     
%     \includegraphics[width=\linewidth]{./fig/overview.pdf}
%     \caption{Overarching Workflow of Executing the DL Program and Building a DL Model}\label{fig:overview}
%     % \xy{Figure improved here}
%     % \vspace{-10pt}
% \end{figure}

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \begin{center}
%     \includegraphics[width=0.5\textwidth]{./fig/cradle.pdf}
%     \caption{Trigger Inputs for Inconsistencies Between DL Frameworks}
%     \label{fig:cradle_demo}
%     \end{center}
%     \vspace{-15pt}
% \end{wrapfigure}


% \begin{figure}
%     \centering 
%     \begin{minipage}[b]{0.48\textwidth} 
%     \centerline{\includegraphics[width=\textwidth]{./fig/cradle.pdf}} 
%     \caption{Trigger Inputs for Inconsistencies Between DL Frameworks}
%     \label{fig:cradle_demo}
%     \end{minipage} 
%     \hfill
%     \begin{minipage}[b]{0.48\textwidth} 
%     \centering%该小页居中排放图片 
%     \centerline{\includegraphics[width=\textwidth]{./fig/audee-2time.pdf}}
%     \caption{An NaN bug Detected by Audee on PyTorch}
%     \label{fig:audee_demo}
%     \end{minipage} 
%     \vspace{-10pt}
% \end{figure}

==> tftex/seca_fig2.tex <==
% \begin{figure}
%     \centering     
%     \includegraphics[width=\linewidth]{./fig/overview.pdf}
%     \caption{Overarching Workflow of Executing the DL Program and Building a DL Model}\label{fig:overview}
%     % \xy{Figure improved here}
%     % \vspace{-10pt}
% \end{figure}

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \begin{center}
%     \includegraphics[width=0.5\textwidth]{./fig/audee-2.pdf}
%     \caption{An NaN bug Detected by Audee on PyTorch}
%     \label{fig:audee_demo}
%     \end{center}
%     \vspace{-15pt}
% \end{wrapfigure}

==> tftex/seca_fig3.tex <==
% \begin{figure}
%     \centering     
%     \includegraphics[width=\linewidth]{./fig/overview.pdf}
%     \caption{Overarching Workflow of Executing the DL Program and Building a DL Model}\label{fig:overview}
%     % \xy{Figure improved here}
%     % \vspace{-10pt}
% \end{figure}

\begin{wrapfigure}{r}{0.4\textwidth}
    \begin{center}
    \includegraphics[width=0.4\textwidth]{./fig/titanfuzz-1times.pdf}
    \caption{An Example PyTorch bug that is only Detected by TitanFuzz.}
    \label{fig:titanfuzz_demo}
    \end{center}
    % \vspace{-15pt}
\end{wrapfigure}

==> tftex/secb_fig1.tex <==
% \begin{figure}
%     \centering     
%     \includegraphics[width=\linewidth]{./fig/overview.pdf}
%     \caption{Overarching Workflow of Executing the DL Program and Building a DL Model}\label{fig:overview}
%     % \xy{Figure improved here}
%     % \vspace{-10pt}
% \end{figure}

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \begin{center}
%     \includegraphics[width=0.5\textwidth]{./fig/cradle.pdf}
%     \caption{Trigger Inputs for Inconsistencies Between DL Frameworks}
%     \label{fig:cradle_demo}
%     \end{center}
%     \vspace{-15pt}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0.4\textwidth}
    \begin{center}
    \includegraphics[width=0.4\textwidth]{./fig/hirgentime.pdf}
    \caption{A Crash on the \texttt{relay.build} of TVM Compiler and was Detected by HirGen.}
    \label{fig:hirgen_demo}
    \end{center}
    % \vspace{-15pt}
\end{wrapfigure}

==> tftex/structure.tex <==
\begin{figure}
    \centering     
    \includegraphics[width=0.95\linewidth]{./fig/structure-new.pdf}
    \caption{Overview of This Paper \todo{Update with RQ or remove it}}\label{fig:structure}
    % \xy{Figure improved here}
    % \vspace{-10pt}
\end{figure}
